Meta Dialogue Policy Learning

Dialog policy determines the next-step actions for agents and hence is central to a dialogue system. However, when migrated to novel domains with little data, a policy model can fail to adapt due to insufficient interactions with the new environment. We propose Deep Transferable Q-Network (DTQN) to utilize shareable low-level signals between domains, such as dialogue acts and slots. We decompose the state and action representation space into feature subspaces corresponding to these low-level components to facilitate cross-domain knowledge transfer. Furthermore, we embed DTQN in a meta-learning framework and introduce Meta-DTQN with a dual-replay mechanism to enable effective off-policy training and adaptation. In experiments, our model outperforms baseline models in terms of both success rate and dialogue efficiency on the multi-domain dialogue dataset MultiWOZ 2.0.

==> algo.tex <==
\begin{algorithm}[t]
\small
\caption{Meta Dialogue Policy Learning}% \textbf{Input:} 
% $\mathcal S = \{\mathcal S_d\}_1^D$: Label combinations\\
% \makebox[1.05cm]{} $\mathcal O = \{\mathcal O_d\}_1^D$: Sentence subcorpora\\
% \makebox[1.05cm]{} $\ell_{max}$: Maximum document length

% \textbf{Output:} A synthetic document
\begin{algorithmic}[1]
\label{algo}
\Function{EnvInteract}{$t$, $\mathcal M$, $B$}  \Comment{Task, memory and number of steps}
\State Initialize number of steps $b \gets 0$
\While {true}  \Comment{A new dialogue episode}
\State Initialize a user agenda with task $t$ and user starts a dialogue with user action $a_u$
\State Generate an initial dialogue state $s$
\While {$s$ is not a terminal state} \Comment{Till the end of an episode}
\State With probability select a random action $a$, otherwise select a = argmax$_{a'}$ $Q(s, a'; \theta_Q)$
\State Execute $a$, and observe user response $a_u$ and reward $r$
\State Update dialogue state to $s\gets s'$
\State Store $(t, s, a, r, a^u , s')$ to $\mathcal M$
\State $b \gets b+1$
\If{$b \geq B$}
\State \Return
\EndIf
\EndWhile
\EndWhile
\EndFunction
\vspace{0.05in}
\renewcommand{\algorithmiccomment}[1]{{\color{red}
\hfill$\triangleright${\textit{ #1}}}}
\Function{MetaPolicyLearning}{}
\State Initialize $Q(s, a; \theta_Q)$ and $Q'(s, a; \theta_{Q'})$ with $\theta_{Q'}\gets\theta_{Q}$  \Comment{Policy network and target network}
\State Initialize experience replay memory $\mathcal M_{\textit{tr}}$ and $\mathcal M_{\textit{ev}}$ using Reply Buffer Spiking (RBS)  \Comment{Dual replay}

\For{$n\gets 1:N$} \Comment{Outer loop for meta-training}
    \State generate $K$ dialogue goals $ \{t_1, ..., t_K\} \text{ where }  t_k=d_k \text{ or } t_k \sim Uniform (\mathcal{T}_{d_k})$
    \State Initialize meta-training loss $\mathcal{L} \gets 0$ 
    \For{$k\gets1:K$} \Comment{Inner loop for task data collection and training}
        \State $\theta' \gets \theta$ and load agent with $\theta'$
        \State \Call{EnvInteract}{$t_{k}$, $\mathcal M_{\textit{tr}}$, $B_{\textit{tr}}$}
        \State Sample random minibatches of $(t_k, s, a, r, s')$ from $\mathcal M_{\textit{tr}}$
        \State Update $\theta'$ via $Z$-step minibatch SGD
        \State \Call{EnvInteract}{$t_{k}$, $\mathcal M_{\textit{ev}}$, $B_{\textit{ev}}$}
        \Comment{Task training data collection}
        \State Sample random minibatches of $(t_k, s, a, r, s')$ from $\mathcal M_{ev}$
        \Comment{Task test data collection}
        \State Forward pass with the minibatches and obtain $\mathcal{L}_{t_k}$
        \State $\mathcal{L} \gets \mathcal{L}+\mathcal{L}_{t_k}$
    \EndFor
    \State Load agent with $\theta_Q$ and update with respect to $\mathcal{L}$ via minibatch SGD
    \State Every $C$ steps reset $\theta_{Q'}\gets \theta_{Q}$ \Comment{Target network update}
\EndFor
\EndFunction
\end{algorithmic}
\end{algorithm}

% \If{$\lvert \mathcal S^{sent} \rvert < C$ } \Comment{Number of domain labels}
%         \State Generate a noisy domain $\epsilon \in \mathcal Y \setminus \mathcal S^{sent}$
%         \State $\mathcal S^{sent} \gets \mathcal S^{sent} \cup \{\epsilon\}$
%     \EndIf

%   \State $\mathcal S^{cdt} \gets \emptyset$; \Comment{A set of candidate domain sets}
   
%   \For{$\mathcal S_d \in \mathcal S$}
%           \If{$\mathcal S_d \in \mathcal S^{sent}$}
%           \State $\mathcal S^{cdt} \gets  \mathcal S^{cdt} \cup \{\mathcal S_d\}$
%           \EndIf
%       \EndFor
           
%     \State $n_{label} \gets \lvert \mathcal S^{cdt} \rvert$\Comment{Number of unused labels}
%     \State $n_{sent} \gets \ell_{max}$ \Comment{Number of sentence blocks}
%     \State $\mathcal L \gets \emptyset$ \Comment{For generated sentences}

%     \For{$\mathcal S_d^{cdt} \in \mathcal S^{cdt}$}
%         \State $\theta = \min(\lvert \mathcal O_d \rvert, n_{sents} +1 -n_{labels}, \frac{2n_{sents}}{n_{labels}})$
%         \State Generate $\ell_d \sim Uniform (1, \theta)$
%         \State Generate $\ell_d$ sentences $\mathcal L_d \subseteq \mathcal O_d$ 
%         \State $\mathcal L \gets  \mathcal L \cup \mathcal L_c$
%         \State $n_{sent} \gets  \ell_{max} - |\mathcal L|$
%         \State $n_{label} \gets  n_{label} -1$
%     \EndFor
% \State $\mathcal L \gets$ \Call{Shuffle}{$\mathcal L$}
% \State \Return $\mathcal L$

==> algo_env_interact.tex <==
\begin{algorithm}
\small
\caption{Experience Collection for Meta Dialogue Policy Learning}% \textbf{Input:} 
% $\mathcal S = \{\mathcal S_d\}_1^D$: Label combinations\\
% \makebox[1.05cm]{} $\mathcal O = \{\mathcal O_d\}_1^D$: Sentence subcorpora\\
% \makebox[1.05cm]{} $\ell_{max}$: Maximum document length

% \textbf{Output:} A synthetic document
\begin{algorithmic}[1]
\label{algo}
\Function{EnvInteract}{$t$, $\mathcal M$, $B$}  \Comment{Task, memory and number of steps}
\State Initialize number of steps $b \gets 0$
\While {true}  \Comment{A new dialogue episode}
\State Initialize a user agenda with task $t$ and user starts a dialogue with user action $a_u$
\State Generate an initial dialogue state $s$
\While {$s$ is not a terminal state} \Comment{Till the end of an episode}
\State With probability select a random action $a$, otherwise select a = argmax$_{a'}$ $Q(s, a'; \theta_Q)$
\State Execute $a$, and observe user response $a_u$ and reward $r$
\State Update dialogue state to $s\gets s'$
\State Store $(t, s, a, r, a^u , s')$ to $\mathcal M$
\State $b \gets b+1$
\If{$b \geq B$}
\State \Return
\EndIf
\EndWhile
\EndWhile
\EndFunction
\end{algorithmic}
\end{algorithm}


==> table_freq.tex <==
% freq
\begin{table}[t]
\centering
\begin{tabular}{lcc}
  \hline
\textbf{Category} & \textbf{Frequency}& \textbf{Domains} \\
\hline
High-Frequency & 11& \texttt{hotel}$^{\ast}$, \texttt{attraction}, \texttt{restaurant}  \\
Middle-Frequency & 7 & \texttt{train}$^{\ast}$, \texttt{taxi} \\
Low-Frequency & 1 & \texttt{police}$^{\ast}$, \texttt{hospital} \\
\hline
\end{tabular}
\caption{\label{tab:dom_freq}Frequency of domains in existing domain orders in MultiWoz. ${\ast}$ denotes target domains.}
\end{table}

==> table_tgt_no_avg.tex <==
%% constrained_tgt
\begin{table}[t]
\tabcolsep=0.12cm
\bgroup
\def\arraystretch{1.0}
\centerline{
\begin{tabular}{l|ccc|ccc|ccc}
\hline
\multirow{2}*{\textbf{Systems}} & \multicolumn{3}{c}{\texttt{Hotel}} & \multicolumn{3}{c}{\texttt{Train}} & \multicolumn{3}{c}{\texttt{Police}}\\
~ & 
\textbf{Success} & \textbf{Reward} & \textbf{Turns} & 
\textbf{Success} & \textbf{Reward} & \textbf{Turns}& 
\textbf{Success} & \textbf{Reward} & \textbf{Turns}\\
\hline
\rowcolor[gray]{0.95}\multicolumn{10}{c}{\textbf{Few-Shot Models}}\\
\hline
\textsc{Dqn-1k} 
&\hspace{1.5ex}0.00	&\hspace{-0.5ex}-55.70	&17.71	&\hspace{1ex}2.15	&\hspace{-1ex}-56.02	&20.60	&100.00	&76.62	&5.38\\
\textsc{Dtqn-1k}
&53.90	&15.06	&11.62	&61.00	&24.84	&10.36	&100.00	&79.28	&2.72\\
\hline
\rowcolor[gray]{0.95}\multicolumn{10}{c}{\textbf{Adaptive Models}}\\
\hline
\textsc{Dqn} 
&36.00	&\hspace{0.5ex}-9.70   &14.90	&32.20	&\hspace{-1ex}-14.53   &15.17	&{100.00} &76.62&	5.38\\
% \textsc{Meta-Dqn}
% &\yumo{28.90} &\yumo{\hspace{-0.5ex}-19.78}   &\yumo{16.46}	&52.40	&12.81	&12.81	&100.00	&79.28	&2.72\\
\textsc{Dtqn}
&\textbf{62.70}   
&\textbf{27.99}  &\hspace{1ex}\textbf{9.25}
&82.65  
&54.80   
&\hspace{1ex}6.38
&{100.00}
&{79.24}
&{2.76}\\
\textsc{Meta-Dtqn}
&{61.90}
&{26.28}   
&{10.00}
&\textbf{87.45}
& \textbf{61.44}   &\hspace{1ex}\textbf{5.50} 
&{100.00}
&{79.24}
&{2.76}\\
\hline
\end{tabular}
}
\egroup
\caption{\label{tab:tgt_single} 
  System performance in the single-domain setting on 2000 dialogues in the target domains. 
%   Success denotes success rate.
  }
\end{table}


%% tgt_cross
\begin{table}[t]
% \tabcolsep=0.11cm
\bgroup
\def\arraystretch{1.0}
\centerline{
\begin{tabular}{l|ccc|ccc}
\hline
\multirow{2}*{\textbf{Systems}} & \multicolumn{3}{c}{\texttt{Hotel}} & \multicolumn{3}{c}{\texttt{Train}}\\
~ & 
\textbf{Success} & \textbf{Reward} & \textbf{Turns} & 
\textbf{Success} & \textbf{Reward} & \textbf{Turns}\\
\hline
\rowcolor[gray]{0.95}\multicolumn{7}{c}{\textbf{Few-Shot Models}}\\
\hline
\textsc{Dqn-1k} 
&\hspace{1ex}0.00	&-50.38	&12.38
&\hspace{1ex}2.15	&-56.02 &20.60\\
\textsc{Dtqn-1k}
&\hspace{1ex}2.55&	-47.77&	12.84	&\hspace{1ex}8.90&	-45.96&	18.64\\
\hline
\rowcolor[gray]{0.95}\multicolumn{7}{c}{\textbf{Adaptive Models}}\\
\hline
\textsc{Dqn} 
&\hspace{1ex}3.90&	-53.74	&20.42
&\hspace{1ex}9.85&	-45.52	&19.34\\
% \yumo{\textsc{Meta-Dqn}} 
% &\hspace{1ex}0.00	&-50.17	&12.18	&\hspace{1ex}4.25&	-53.13&	20.23\\
\textsc{Dtqn}
&\hspace{1ex}4.15   &-53.32 &20.30
&15.40	&-37.93	&18.41\\
\textsc{Meta-Dtqn}
&\textbf{11.45}	&\textbf{-43.68} &\textbf{19.42}	
&\textbf{19.30}	&\textbf{-32.81}	&\textbf{17.97}\\
\hline
\end{tabular}
}
\egroup
\caption{\label{tab:tgt_cross} 
  System performance in the composite-domain  setting on 2,000 dialogues in the target domains. 
%   Success denotes success rate.
  We show results in \texttt{Hotel} and \texttt{Train} as \texttt{Police} has only single-domain dialogue goal.
}
\end{table}
